Automated Theorem Proving in Intuitionistic Propositional Logic by Deep Reinforcement Learning

The problem-solving in automated theorem proving (ATP) can be interpreted as a search problem where the prover constructs a proof tree step by step. In this paper, we propose a deep reinforcement learning algorithm for proof search in intuitionistic propositional logic. The most significant challenge in the application of deep learning to the ATP is the absence of large, public theorem database. We, however, overcame this issue by applying a novel data augmentation procedure at each iteration of the reinforcement learning. We also improve the efficiency of the algorithm by representing the syntactic structure of formulas by a novel compact graph representation. Using the large volume of augmented data, we train highly accurate graph neural networks that approximate the value function for the set of the syntactic structures of formulas. Our method is also cost-efficient in terms of computational time. We will show that our prover outperforms Coq's $\texttt{tauto}$ tactic, a prover based on human-engineered heuristics. Within the specified time limit, our prover solved 84% of the theorems in a benchmark library, while $\texttt{tauto}$ was able to solve only 52%.

==> 4.1-library.tex <==
% \subsection{Problem Library}

%We generated formulas by a random generation algorithm for data libraries.
%We describe the algorithm in Algorithm~\ref{alg:formula} in Supplementary Material.
%Given a ``desired'' length parameter $n$, we recursively generate a syntax tree from top to bottom.
%When we generate a leaf node, we uniformly choose a propositional variable from candidates at random.
%When we generate an intermediate node, we randomly choose a logical symbol.
%A generated formula has length between $n/2$ and $n$.

%In our experiment, we generated $D_\mathrm{train}$ with randomly sampled parameters $n \in [50, 400]$ and $m \in [2, 20]$.
%We generated $D_\mathrm{exam}$ with $n=500$ and $m \in [2,20]$.
%Since generated formulas are not necessarily provable in IPL, we checked their validity using an existing IPL prover.
%We generated 2000 IPL theorems for $D_\mathrm{train}$ and 1000 for $D_\mathrm{exam}$.
